Community-based anomaly detection using spectral graph filtering

Several applications have a community structure where the nodes of the same community share similar attributes. Anomaly or outlier detection in networks is a relevant and widely studied research topic with applications in various domains. Despite a significant amount of anomaly detection frameworks, there is a dearth on the literature of methods that consider both attributed graphs and the community structure of the networks. This paper proposes a community-based anomaly detection algorithm using a spectral graph-based filter that includes the network community structure into the Laplacian matrix adopted as the basis for the Fourier transform. In addition, the choice of the cutoff frequency of the filter considers the number of communities found. In computational experiments, the proposed strategy, called SpecF, showed an outstanding performance in successfully identifying even discrete anomalies. SpecF is better than a baseline disregarding the community structure, especially for networks with a higher community overlapping. Additionally, we present a case study to validate the proposed method to study the dissemination of COVID-19 in the different districts of S\~ao Jos\'e dos Campos, Brazil.

==> chapters/anomaly.tex <==
The anomaly studied in this paper is defined as a vertex $v_i$ whose signal $f(v_i)$ is far from the expected standard found in the community to where  $v_i$ belongs. In this case, most of the signal’s energy is concentrated in the low-frequency signals of the Fourier transform. A node with a signal value that considerably differs from the neighborhood average will probably be anomalous. 

This type of anomaly is observed, for example, in temperature sensor networks, in which neighboring sensors are expected to have close measured values. In this case, a potential anomaly is a sensor measurement that deviates significantly from the values sensed by neighboring nodes, such as a sensor failure. In protein-protein interaction networks, expression levels of neighboring nodes that represent proteins belonging to the same biological process usually vary proportionately. For example, if the expression level of a protein increases, other proteins that belong to the same biological process usually have their expression level increased or decreased accordingly. In this case, where proteins from the same biological process generally belong to the same community, a potential anomaly is a node with a variation of expression level significantly different from the nodes in the same community, e.g., a protein involved in cancerous processes.

%PAREI AQUI  we define that the set of vertices whose signal value has undergone a greater correction after the filtering process is a set whose vertices are more likely to be anomalous.
%
We hypothesize that the attenuation of the magnitude of the signal spectrum at high frequencies can correct the abrupt variations that define the studied anomalous behavior. Thus, in this paper, we suggest that vertices whose signal value needed a substantial correction after the filtering process are more likely to be anomalous. In line with this, to find the anomalous vertices, this paper introduces \textit{SpecF}, which is a strategy that uses a low-pass filter to attenuate the magnitude of the high frequencies of the spectrum $\hat{\mathbf{f}}$ of a signal $\mathbf{f}$. The inverse Fourier transform, defined in Equation \eqref{eq:inversefourier}, is applied to the filtered spectrum to obtain a filtered signal $\mathbf{f'}$. We compare the filtered signal $\mathbf{f'}$ with the original signal $\mathbf{f}$ to determine to which vertices the signal value has been severely attenuated, to obtain the set of potentially anomalous vertices. To evaluate the proposed strategy, this paper also introduces an approach to generate synthetic anomalous signals similar to the signals considered in our hypothesis. In the next section, we discuss the details of the anomaly generator and the proposed anomaly detection algorithm.

\subsection{Expanded Adjacency Matrix}\label{expand_matrix}

Let $W \in \mathbbm{R}^{n\times n}$ be the so-called expanded matrix that incorporates the community structure of a graph to represent the pairwise relationship between vertices $v_i$ and $v_j \in V$, referred to as $w_{ij}$. The values $w_{ij}$ are defined in Equation \eqref{case:case1},  where $c_{v_i}$ is the community where vertex $v_i$ belongs.%In this paper, we adopted an expanded adjacency matrix $W$ to include community structure in the matrix used for the Fourier transform. The values $w_{ij}$ are defined as

\begin{equation}\label{case:case1}
w_{ij}=
\begin{cases}
    5,& \text{if $v_i$ and $v_j$ are neighbors and $c_{v_i}$ = $c_{v_j}$}\\
    3,& \text{if $v_i$ and $v_j$ are neighbors and  $c_{v_i} \neq c_{v_j}$}\\
    1,& \text{if $v_i$ and $v_j$ are not neighbors and  $c_{v_i} = c_{v_j}$}\\
    0,              & \text{otherwise}
\end{cases}
\end{equation}

According to the definition of the expanded matrix, if vertices $v_i$ and $v_j$ are adjacent and in the same community,  $w_{ij}$ will receive the highest weight, the value 5. If they are adjacent but belong to distinct communities, $w_{ij}$ will receive the intermediary value 3.  If the two vertices are not adjacent but are in the same community, $w_{ij}$ will receive a value of 1. As a consequence, an explicit affinity between these vertices is defined in such a matrix. Other edges assume a null weight and are disregarded.% This expanded adjacency matrix can be seen as the insertion of new edges in  $G$, \textcolor{red}{ensuring that all vertices in a same community are connected by an  edge.}
%This expanded adjacency matrix can be seen as the insertion of new edges in  $G$, so that all vertices that belong to the same community are connected by a weighted edge.

\subsection{Normal Signal Generator} \label{cap:generator}

Let $G^c$ be a graph whose nodes $v^c_i$ represent communities $c_i$ of $G$ and the edge weights $w^c_{ij}$ are defined as the number of edges between communities $c_i$ and $c_j$. To define a signal $S^c$, the nodes of $G^c$ are sorted according to the sum of the edges' weights $w^c_{ij}$ and $s_i^c$ is then defined as  

%The first stage of the generator creates a signal $S$ where each element $s_i^c \in S^c$ represents the average value of the signal $S$ for nodes that belong to a community $c$ of $G$. Considering a graph $G^c$, where nodes $v^c_i$ of $G^c$ represents communities $c_i$ of the original graph $G$ and an edge weight $w^c_{ij}$ of $G^c$ is defined as the number of edges between communities $c_i$ and $c_j$ of $G$. The nodes $v_i^c$ are ordered according to the sum of the edges $w^c_{ij}$ and $s_i^c$ is defined as

\begin{equation} \label{eq:signal_sc}
s_i^c = \sum_{\forall v^c_j \in \mathcal{N}_{i}^c} w^c_{ij} \times (i+1)
\end{equation} 


\noindent where $\mathcal{N}_{i}^c$ is the set of nodes adjacent to $v_i^c$.%, and $i$ is the index of $v_i^c$ after sorting. 

To properly evaluate the anomaly detection strategy proposed in this paper, we developed an artificial signal generator. The generator produces a synthetic signal $S$ similar to the signal observed in the investigated applications. As a result, it creates signals whose values for nodes of the same community are similar. 

Algorithm \ref{alg:algoritmo2} describes the process employed by the generator to obtain the signal $S$ from a graph $G$ and a given signal $S^c$, with elements defined by Equation \eqref{eq:signal_sc}. First, all nodes are marked and an auxiliary $n$-dimensional vector $S^x$ is initialized as empty. For every community $c_i$ of $G$, the algorithm assigns the value of $s_i^c$ to the position of $S^x$ that corresponds to the highest degree node in community $c_i$. In the case of a tie, a node is randomly selected among the highest degree nodes.  These nodes are regarded as community heads. Then, the algorithm starts a propagation process from the community heads. Each node propagates a percentage of its value to its neighbors. This percentage is lower (10\%) if the nodes involved belong to different communities, and higher (at least 25\%) if they are in the same community. For nodes from the same community, this percentage also depends on their degree, so that nodes with higher degrees have a greater influence on lower degree nodes. After the propagation process, every node that propagated values has its value reduced by 5\%. This process is repeated until all nodes have propagated a number of their signal values. The last step consists of a normalization process to define the signal of each node as that considers the weight of the edge between neighbor nodes to carry out a weighted average.


\begin{algorithm}[!h]
\small
\KwData{A graph $G$, a signal $S^c$, a partition $\mathcal{C}$ }
\KwResult{A signal $S$}

Mark all nodes\;
$S^x \leftarrow \emptyset$\;

\ForAll{ community $c_i\in G$}{
    $v_k \leftarrow$ the highest degree node of $c_i$\;
    $s^x_k \leftarrow s^c_i$\;
    Unmark $v_i$\;
}

%$S^x\leftarrow$ An normal distribution with the mean and standard deviation of $S^c$\;
%$L$ $\leftarrow$ Neighbors of all unmarked vertices\;

Create a list $F$ with all unmarked nodes sorted by index values\;
\While{there is a node in $F$}{ 
    \textcolor{black}{Select the first node $v_i$ from $F$}\;
    \ForAll{$v_j\in \mathcal{N}_i$ }{
        $t \leftarrow 0.1$\;
        \If{$v_i$ and $v_j$ are in the same community}{
            $mt \leftarrow  \ddfrac{degree(v_i)}{degree(v_j) + degree(v_i)}$\;
            $t \leftarrow max(0.25, mt)$\;
        }
        $s^x_j \leftarrow s^x_j + (s^x_i \times t$)\;
        $s^x_i \leftarrow s^x_i \times 0.95$\;
        \If{$v_j$ is marked}{
            Unmark $v_j$ and include $v_j$ at the end of $F$\;
        }
    }
    %$x\leftarrow$ Mean of $S_k$ for all unmarked neighbor $v_k$ of $v_i$\;
    %$S[i]\leftarrow$ $S^x$ value closest to $x$\;
    Remove $v_i$ from $F$\; % and remove $S[i]$ from $S^x$\;
    %unmark $v_i$ and include $v_i$'s marked neighbors in $L$\;
}
\ForAll{$v_i\in G$}{
    $s_i \leftarrow   \frac{\sum_{j=1}^n w_{ij}\times s_j^x}{\sum_{j=1}^n w_{ij}}$\;
}
\caption{\textsc{Normal Signal Generator}}
\label{alg:algoritmo2}
\end{algorithm}


%among the nodes of each community $c_i$ in a LFR network with 500 nodes, generated using the parameters defined in Table \ref{tab:parameters}. 
Figure \ref{fig:gerador2} presents box-plots of the values of the $S$ signal, obtained through Algorithm \ref{alg:algoritmo2} applied to a 500-node LFR network \citep{Lancichinetti2009} with the parameters defined in Table \ref{tab:parameters} and low overlapping between communities (mixture degree 0.1).  The network has 10 planted communities. Section~\ref{subsec:artificial} describes the parameters and the software to generate the networks. We show a box-plot for each of the expected communities, sorted in increasing order of intra-community average signal.
%The communities $c_i$, defined in the expected partition of the artificial LFR network, are ordered according to the average signal for the nodes of that community.
Through Figure \ref{fig:gerador2}, it is possible to notice that, although the average value of signal $S$ in each community is different, vertices of the same community have similar values.


% \begin{figure}
% 	\centering
% 		\includegraphics[scale=.4]{figs/box_GLOBAL.eps}
% 	\caption{Box-plots of $S$ for each community of $G$.}
% 	\label{fig:gerador2}
% \end{figure}

\begin{figure}[h!t]
\center

\input{tikz/box_GLOBAL.tex}

\caption{Box-plots of $S$ for each community of $G$.}
\label{fig:gerador2}
\end{figure}


%PAREI AQUI
\subsection{Anomaly Generator}\label{subsec:gerador}

In addition to the normal signal generator, we hereby introduce a strategy to create anomalous signals in an attributed network. 

For such, consider a signal $S$ of a graph $G$. We generate an anomalous signal $B$ from signal $S$ by increasing the value of $s_{i}$ in some vertices of $G$. This process is detailed in Algorithm \ref{alg:algoritmo3}, which randomly selects a set of nodes to corrupt. The anomaly intensity $\theta$ defines how much greater the value of an anomalous node will be when compared to the rest of the community. An anomaly intensity value of $0.1$, for example, means that an anomalous node will have a signal value between 5\% and 10\% higher than the largest signal value of that community.

\begin{algorithm}[!h]
\small
\KwData{A graph $G$, a normal signal $S$, percentage of anomalies $AN$, anomaly intensity $\theta$}
\KwResult{An anomalous signal $B$}
$B \leftarrow$ Create a copy of $S$\;
$P \leftarrow$ Randomly select a set with $AN\%$ of distinct vertices of $G$\;
\ForAll{vertex $v_i$ in $P$}{ 
    $max\leftarrow$ Highest value of $S$ among nodes in $c_{v_i}$\;
    $tax \leftarrow$ Random value between $\frac{1}{2}\theta$ and $\theta$\;
    $b_i$ = $max \times (1 + tax)$\;
}
\caption{\textsc{Anomalous Signal Generator}}
\label{alg:algoritmo3}
\end{algorithm}

Figure \ref{fig:anomalia1} illustrates the values of an anomalous signal $B$ at each node highlighting the anomalies (when `Anomaly' is 1), ordered by their community average, as in Figure \ref{fig:gerador2}. It is possible to see that, when sorted by the community average, the anomalous nodes become more evident. However, they are within the mean and standard deviation values when considering the complete signal, which makes them difficult to find using techniques that do not consider the network community structure.

% \begin{figure}
% 	\centering
% 		\includegraphics[scale=.45]{figs/anomalous_ordered.eps}
% 	\caption{Example of an anomalous signal $B$.}
% 	\label{fig:anomalia1}
% \end{figure}

\begin{figure}[htbp]
\center

\input{tikz/anomalous_ordered.tex}

\caption{Example of an anomalous signal $B$.}
\label{fig:anomalia1}
\end{figure}

\subsection{Low-pass Filter and the Cut-off Frequency}

In GSP theory, the first $k$ eigenvalues of $L$ correspond to the $k$-lowest frequencies in the spectrum of a signal. Low frequencies carry the information of signals that vary little across the nodes of the network. Moreover, our strategy focuses on a signal whose intra-community variation is expected to be low. Therefore, we propose to choose the number of communities $k$ in the network as the cut-off frequency, so that $\lambda_{cut} = \lambda_k$. A low-pass filter, as defined in Section \ref{sec:filter}, attenuates the magnitude of high-frequency signals and keeps low frequencies unchanged. In this case, a high-frequency is defined as a frequency $\lambda_l$ higher than the cut-off frequency $\lambda_{cut}$, that is, $\lambda_l > \lambda_{cut}$.

In cases where the expected partition is known beforehand, the choice of $\lambda_k$ is trivial, since $k$ is the number of communities. On the other hand, when the number of communities is unknown,  two approaches to estimate the number of communities in the network can be used. The first approach consists in applying a community detection algorithm to the network to estimate the number of the communities $k$ -- algorithms that do not require the number of communities to be informed beforehand. The second approach comes from graph theory and consists of finding the value of $k$ by analyzing the eigenvalues of $L$ and choosing $k$ so that $\lambda_1, ..., \lambda_k$ are very small, but $\lambda_{k+1}$ is relatively large. In spectral graph theory, when a graph has $k$ completely disconnected components, the first $k$ eigenvalues of $L$ will have the value 0 and then there is a gap to the eigenvalue in position $k+1$ \citep{VonLuxburg2007AClustering}.


% Figure \ref{fig:filtro1} illustrates the frequency response of a low-pass filter, as defined in Section \ref{sec:filter}, considering the cut-off frequency $\lambda_{cut}$ = $\lambda_k$, where $k$ is the number of inherent communities. In this case, where $k = 10$, it is possible to notice that the magnitude of the spectrum for $\lambda_l \leq \lambda_{cut}$ remains unchanged, while it is considerably attenuated for $\lambda_l > \lambda_{cut}$.
  
% \begin{figure}
% 	\centering
% 		\includegraphics[scale=.45]{figs/filtro1.eps}
% 	\caption{Frequency response of the filter.}
% 	\label{fig:filtro1}
% \end{figure}


\textit{SpecF} uses the Fourier transform, defined in Equation \eqref{eq:fourier}, to calculate the spectrum $\hat{B}$ of signal $B$. The $\hat{B}$ spectrum is submitted to the proposed low-pass filter to obtain a filtered spectrum $\hat{B}'$. Then, the inverse Fourier transform is applied in $\hat{B}'$ to obtain a filtered signal $B'$, illustrated in Figure \ref{fig:anomalia2}.

\textcolor{black}{A comparison of the signal $B'$ with the signal $B$ allows us to observe that} the groups of vertices are more cohesive \textcolor{black}{ in signal $B'$}, demonstrating that the filter made the signal values even closer to nodes from the same community. In addition, the anomalies, which previously diverged from other nodes in the same community, are now within the expected standard.

% \begin{figure}
% 	\centering
% 		\includegraphics[scale=.45]{figs/anomalous_ordered2.eps}
% 	\caption{Example of a filtered anomalous signal $B'$.}
% 	\label{fig:anomalia2}
% \end{figure}

\begin{figure}[htbp]
\center

\input{tikz/anomalous_ordered2.tex}

\caption{Example of a filtered anomalous signal $B'$.}
\label{fig:anomalia2}
\end{figure}

\subsection{Potentially Anomalous Nodes}\label{subsec:anomalous}

Figure \ref{fig:anomalia2} shows the ability of the \textit{SpecF} to correct anomalies and normalize the values of a signal according to the network's community structure. We compared the filtered signal $B'$ with the original anomalous signal $B$ to identify in which nodes the correction of the signal was more significant. The intuition behind this idea is that, if anomalous nodes differ from what is expected for their community, the normalization applied considering the filter will be more intense in these nodes. Thus, when identifying these nodes, a set of nodes with the greatest anomalous potential is also detected. For such, we define a  signal  $Y = \abs{B - B'}$. In general, vertices $v_i$ with a high $y_i$ value are more likely to be anomalous and we can adopt the vector $Y$ as an abnormality quantifier. To classify the nodes as anomalous or normal in a binary way, we can consider a threshold to distinguish which $y_i$ values are considered normal and which are identified as abnormal observations. The threshold values employed in \textit{SpecF} are regarded for each community taking the mean and standard deviation of $Y$ into account, as presented in Equation~\eqref{eq:threshold}. 

\begin{equation}
    TD(Y, c_k) = \ddfrac{mean(Y, c_k) + 2std(Y, c_k)}{max(Y, c_k)}
    \label{eq:threshold}
\end{equation}



\noindent where $c_k$ is a community of $G$; $mean(Y, c_k)$, $std(Y, c_k)$ and $max(Y, c_k)$ are, respectively, the mean, standard deviation and  maximum of the values of $Y$ that represent the nodes of community $c_k$. Figure \ref{fig:anomalia3} illustrates the relation between $y_i$ values and the vertices of a network. Moreover, it presents  the threshold values $TD(Y, c_k)$ -- dotted curve --  that separate  anomalous nodes from  normal nodes. It is possible to notice that the vast majority of nodes above the red curve are true positives and, therefore, are in the set of anomalous nodes defined by the generator. On the other hand, most of the nodes below the red curve are true negatives and, therefore, are labeled normal. There are also false positives and false negatives and they are usually close to the threshold curve.

% \begin{figure}
% 	\centering
% 		\includegraphics[scale=.45]{figs/anomalous_type.eps}
% 	\caption{Example of a signal $Y$ and the threshold.}
% 	\label{fig:anomalia3}
% \end{figure}


\begin{figure}[htbp]
\center

\input{tikz/anomalous_type.tex}

\caption{Example of a signal $Y$ and the threshold.}
\label{fig:anomalia3}
\end{figure}

In the next section, we present the computational experiments performed to evaluate the efficiency of \textit{SpecF}.

==> chapters/case.tex <==
We performed an experiment with real data to validate the performance of the anomaly detection strategy proposed in this paper. The data set used in the experiment contains the number of daily  COVID-19  cases in each of the districts of São José dos Campos, an upstate city of São Paulo - Brazil. We model the data as a graph $G$, where the nodes represent districts of the city. A pair of nodes $v_i$ and $v_j$ is connected if the distance between the corresponding districts is less than 5 km. In this case, the weight $w_{ij}$ of the edge is proportional to the distance between districts represented by nodes $v_i$ and $v_j$. Figure \ref{fig:graph} illustrates the graph $G$, where the nodes were colored according to their communities (meaning that nodes with the same color belong to the same community). The graph $G$ has 366 nodes and the community structure of the network was identified using a community detection algorithm named Louvain \citep{Blondel2008FastNetworks}. The Louvain method is a benchmark community detection heuristic that identifies the community structure through the modularity optimization  \citep{Newman2004FindingNetworks}.

\begin{figure}
	\centering
		\includegraphics[scale=0.12]{figs/graph.eps}
	\caption{Graph representing the districts of São José dos Campos, SP, Brazil.}
	\label{fig:graph}
\end{figure}

We used data collected from March 5, 2020 to March 25, 2021, totaling 385 days (equivalent to 55 weeks). For each week, we consider the subgraph formed exclusively by the districts that had at least 2 cases in the previous and current weeks. Thus, for each week, the number of nodes and the community structure of the graph are modified due to the removal of some nodes that represent districts that did not have a sufficient number of cases in the analyzed weeks. We define the signal $B^{(d)}$ as the weekly variation in the number of COVID-19 cases, where $b_i^{(d)}$ is the ratio between the sum of the total number of cases registered between days $d-7, d-6, \ldots, d-1$ and days $d, d+1, \ldots, d+6$ in the district represented by node $v_i$. We applied the proposed anomaly detection strategy in signal $B^{(d)}$ to identify anomalies in the weekly variation of cases. Our hypothesis is that if the number of cases in a given district increases, the number of cases in adjacent districts must increase as well. In this way, we can apply\textit{SpecF} to identify neighbor districts whose variation in the number of cases differs from a given district in a certain week.

The upper part of Figure \ref{fig:hitmap} illustrates the weekly variation in the number of cases in each of the districts. The 366 different districts are represented by the y-axis whereas the x-axis represents the weeks. The signal corresponding to week 2, for example, is represented by $B^{(14)}$, since we calculate $d$ by multiplying the week number by 7. The intensity of the colors represents the weekly variation in the number of cases. The redder the greater the increase in the weekly number of cases. We apply the strategy presented in Section \ref{subsec:anomalous} to find the $Y^{(d)}$ signal that stores the abnormality of the nodes. The lower part of Figure \ref{fig:hitmap} illustrates the abnormality in the variation in the number of cases for each district. It is possible to notice that the amount of light dots at the bottom is considerably smaller. This is because the proposed strategy filters the signal and highlights the abnormalities, so that only potentially anomalous variations are maintained in the $Y^{(d)}$ signal.

% \begin{figure}
% 	\centering
% 		\includegraphics[scale=0.55]{figs/hitmap.png}
% 	\caption{Weekly variation in the number of cases in each of the districts of São José dos Campos, SP, Brazil.}
% 	\label{fig:hitmap}
% \end{figure}

\begin{figure}[h!t]
\center

\input{tikz/hitmap.tex}

\caption{Weekly variation in the number of cases in each of the districts of São José dos Campos, SP, Brazil.}
	\label{fig:hitmap}
\end{figure}


To validate our hypothesis and attest to the veracity of the obtained result, we compared the values of the nodes identified as anomalous with the values of the other nodes of the same community for every day $d = \{0,7,14, \ldots,378, 385\}$. For example, if $y_i^{(d)}$ is pointed out as an anomaly, it means that the variation in the number of cases between the days $d-7,d-1$ and $d,d+6$ in the district represented by node $v_i$ differs from the standard of the community to which $v_i$ node belongs. 

This behavior is best seen in Figure \ref{fig:map}, which illustrates a map with the weekly variation in the number of cases in the districts, with a single anomaly. Shades closer to blue represent a drop in the number of cases, while shades closer to yellow represent an increase in the total of COVID-19 cases. It is possible to observe that most districts experience a reduction in the number of cases, while only one district has an increase. This increase is considered an abnormal incident since the adjacent districts have the number of COVID-19 cases reduced. 

\begin{figure}
	\centering
		\includegraphics[scale=.24]{figs/map.png}
	\caption{Heat map with the weekly variation in the number of cases in each of the district of São José dos Campos, SP, Brazil.}
	\label{fig:map}
\end{figure}

A total of 117 values $y_i^{(d)} $ were identified as anomalous. 94.9\% of these anomalies have the same characteristic: the node identified as anomalous in a time window was the only one that had an increase in the number of cases in its community. Figure \ref{fig:boxplot} shows this behavior for a sample of 50 of the 117 anomalies identified. Each box-plot illustrates the variation values of nodes from the same community to which the anomalous node belongs. The variation values of the anomalous nodes are highlighted in blue dots. The anomalous node presents an increase in the number of COVID-19 cases, in contrast to the other nodes of the same community, that showed a reduction in the number of cases.

% \begin{figure}
% 	\centering
% 		\includegraphics[scale=0.3]{figs/boxplot.eps}
% 	\caption{Box-plots of the weekly variation in the number of COVID-19 cases considering communities with anomalous nodes.}
% 	\label{fig:boxplot}
% \end{figure}


\begin{figure}[h!t]
\center

\input{tikz/boxplot.tex}

\caption{Box-plots of the weekly variation in the number of COVID-19 cases considering communities with anomalous nodes.}
	\label{fig:boxplot}
\end{figure}

We have identified that new anomalies usually occur in districts that are adjacent to districts where abnormal variations were observed in the previous two weeks. In 80.3\% of the cases, if a node $v_i$ is indicated as anomalous in the signal $y_i^{(d)}$, then there is a node $v_j$, neighbor of $v_i$, that is pointed out as anomalous in the signal $y_j^{(d-7)}$ or $y_j^{(d-14)}$, where $d\geq 14$. The results obtained in this case study indicate that our hypothesis was correct. The proposed strategy can identify nodes whose characteristics differ from the others from the same community, even in real-world scenarios. Furthermore, it shows that the anomaly "walks" through the network, such that an anomalous node hits adjacent nodes that become anomalous a few weeks later.

==> chapters/conclusions.tex <==
This paper proposed a method to detect anomalies in signals indexed by graphs, called \textit{SpecF}. \textit{SpecF} uses an extended Laplacian matrix that considers the community structure as the basis for the Fourier transform and a low-pass filter designed to attenuate high frequencies in the signal spectrum. The proposed filter uses as cut-off frequency the eigenvalue whose position is the number of communities in the network. This position can be passed as a parameter or automatically calculated through eigenvalue analysis of the adopted matrix.

Computational experiments attest to the accuracy of \textit{SpecF} in the task of detecting anomalies. Moreover, the automatic calculation of the cut-off frequency using the network community structure makes the method independent of parameters and more robust for dealing with real-world networks. In addition, the experiments show that the proposed method performed better when adopting the expanded adjacency matrix $W$ in the Fourier transform instead of the adjacency matrix $A$.

The results suggest that \textit{SpecF} is an interesting solution to detect anomalies based on signals indexed by graphs. More specifically, the method can successfully identify nodes in the network whose signal value differs from the expected according to the community where they belong. Therefore, the proposed method effectively finds anomalies in signals whose expected variation is low in nodes from the same community.

Besides, a case study was presented to validate the proposed strategy. It consists of data related to the number of COVID-19 cases in the different districts of São José dos Campos, an upstate city of São Paulo, Brazil. We identified districts whose number of cases increased significantly while neighboring districts showed a reduction in the number of cases in the same week. We evaluated if the number of COVID-19 cases in a district in a given week is abnormally high or low. The number of COVID-19 cases in some neighbor districts in the past one or two weeks is also anomalous in most of the cases. This gives evidence that the uncontrolled dissemination of the virus occurs following a ``path'' in the city. 


==> chapters/experiments.tex <==

This section presents three experiments carried out to attest to the efficiency of the anomaly detection method proposed in this paper. In the first experiment, we assess the behavior of \textit{SpecF} by varying the number of anomalies present in the network. The second experiment analyzes \textit{SpecF} when faced with variations in the intensity of the anomalies. Finally, the third experiment evaluates the effectiveness of the strategy in multiple executions with varied parameter values. Before going into detail about the experiments, we discuss the evaluation metrics employed and the networks used.

\subsection{Artificial Networks}\label{subsec:artificial}

A set of artificial networks was generated using the software introduced in \citep{Lancichinetti2009}. We refer to the generated networks as LFR networks. By using this software, we created a set of undirected and unweighted benchmark graphs, with heterogeneous distributions of node degree and community sizes. The mixture degree of the communities reflects how well separated the communities are since a mixture parameter specifies the amount of inter-community edges. Therefore, low values for the mixture parameter produce networks with a more evident division in communities. The nodes of the LFR networks have an average degree $d_G$ of 10 and a maximum degree $max$ $d_G$ of 50. The parameters related to the exponent of the distribution of degrees (neg. exp. $d_G$) and communities' vertex count (neg. exp. $\mid c\mid$) are  2 and 1, respectively. Moreover, the mixture parameter was set to be valued between 0.1 and 0.8, with a step size of 0.1.  Table \ref{tab:parameters} summarizes the parameters used to generate the networks. 

From the LFR networks, we generated normal signals and distributed them over the vertices of the network, according to the methodology discussed in  Section~\ref{cap:generator}. The anomalies were inserted in the networks by modifying the signals, according to the strategy introduced in Section \ref{subsec:gerador}.%These normal signals were used, through the generator introduced in Section \ref{subsec:gerador}, to generate the anomalies that will be used in the computational experiments used in that section.

Figure \ref{fig:lfr_network} illustrates an LFR network with 1000 vertices colored according to the signal values. The bluer a node, the higher its signal value. On the other hand, the redder the nodes, the lower their signal values. Larger nodes are those with a higher number of neighbors. The vertices are separated into different groups that represent the communities to which they belong. One may observe that intra-community vertices have similar colors, for example. However, there are some anomalous vertices, like the blue ones, that subtly clash with the standard of the vertices of their community.

\begin{center}
\begin{table}[t]
\caption{Parameters employed to generate the LFR  networks and the normal/anomalous signal.}
\label{tab:parameters}
\begin{tabular}{@{} *5l @{}}    \toprule
\emph{Parameter} & \emph{Values} \\\midrule
 $n$  & 500 and 1000\\
 $\mu$ (mixture parameter) & 0.1, 0.2, \ldots, 0.8\\
 av. $d_G$ & 10 \\
 max $d_G$ & 50 \\
 neg. exp. $d_G$ & 2 \\
 neg. exp. $\mid c\mid$ & 1\\
 min/max vertex count in communities & 20/100 \\\bottomrule
 \hline
\end{tabular}
\end{table}
\end{center}

\begin{figure}
	\centering
		\includegraphics[scale=.12]{figs/plot_with_anomaly.png}
	\caption{Example of an LFR network with anomalies.}
	\label{fig:lfr_network}
\end{figure}

\subsection{Evaluation Metrics}

We used some classic measures to evaluate and interpret the results obtained by \textit{SpecF}. 

The Receiver Operating Characteristic curve, or ROC curve, summarizes the trade-off between the false positive rate and true positive rate (also known as recall). The ROC curve allows us to compare different models directly, and the area under the curve (AUC) can be used as a model quality quantifier. On the one hand, a random classifier, for example, could be represented by a diagonal curve that has an area of 0.5, starting at the bottom left and ending at the top right of the ROC space. On the other, a curve that starts in the lower-left corner, moves up to the upper left corner, and then advances to the upper right corner, adding up to an area of 1 would represent an ideal classifier.

%Although the ROC curve is a widely adopted metric, it should be used when there is a balanced amount of samples in the data set \citep{Fawcett2004, Davis2006}. \textcolor{red}{O artigo que você cita, muito conhecido na área de AM, diz o contrário do que você está afirmando sobre ROC: In addition to being a generally useful performance graphing method, they have properties that make them especially useful for domains with skewed class distribution and unequal classification error costs. Melhor não entrar nesse mérito...} \textcolor{red}{In cases where  binary classifiers are applied to data with unbalanced distribution of samples over the classes}, the precision-recall curve is pointed out as a more informative metric \citep{Saito2015TheDatasets}. This is the case of the application studied in this paper. 

In cases of binary classification problems with a skewed distribution of numbers of observations per class,  \cite{Saito2015TheDatasets} point out the precision-recall curve as a more informative metric. Since our application is characterized by a skewed distribution (there are far more normal cases than anomalies), we also employ a precision-recall curve in the evaluation of the anomaly detection performance. The precision-recall curve is similar to the ROC curve, but it compares precision with recall for different thresholds. Precision corresponds to the proportion of true positives concerning the sum of true positives and false positives. A random classifier, in this case, is represented by a horizontal line with a value proportional to the number of positive cases in the data set. An efficient classifier, on the other hand, would be represented by a line that approaches the upper right point. Again, the Area Under the Precision-Recall Curve (AUC-PR) can be used as a quantifier of the classification model's ability, also called Average Precision (AP) \citep{Saito2015TheDatasets}. % AP summarizes a precision-recall curve as the weighted average precision achieved at each threshold, with the increase in recall from the previous threshold used as the weight \cite{Saito2015TheDatasets}.


\subsection{Experiment I}\label{subsec:experiment1}

The first experiment seeks to evaluate the performance of \textit{SpecF} by varying the number of anomalies and keeping the intensity $\theta$ at 5\%.  For this experiment, we tested \textit{SpecF} with different percentages of anomalies in data ($AN$) for an LFR network with 500 nodes, mixture parameter $\mu = 0.1$ and the other parameters following the values shown in Table \ref{tab:parameters}. We performed 10 different runs with each combination of parameters. Table \ref{tab:experiment1} presents the mean and standard deviation of the AUC-ROC and PR values considering the 100 independent runs, when a standard adjacency matrix is used. These results show that the performance of \textit{SpecF} improves as $AN$ increases. Similarly, Table \ref{tab:experiment1b} presents the results of the same experiment, but using the expanded adjacency matrix $W$ instead of the adjacency matrix $A$ to calculate the Fourier transform defined in Section \ref{sec:fourier}. A comparison of the results with both matrices reveals that in all cases the anomaly detection strategy performed much better using the expanded adjacency matrix $W$.

%Figures \ref{fig:roc_1} and \ref{fig:pr_1} illustrate, respectively, the ROC and precision-recall curves of this experiment.

\begin{center}
\begin{table}[t]
\caption{Results of experiment I using the  standard  adjacency matrix}
\label{tab:experiment1}
\begin{tabular}{@{} *5l @{}}    \toprule
\emph{\% of anomalies (AN)} & \emph{AUC ROC} & \emph{AP} \\\midrule
$1\%$  &  0.899 +/- 0.042 & 0.511 +/- 0.099 \\
$5\%$  &  0.936 +/- 0.029 & 0.639 +/- 0.098 \\
$10\%$  &  0.928 +/- 0.023 & 0.704 +/- 0.067 \\
$15\%$  &  0.953 +/- 0.017 & 0.808 +/- 0.050 \\
$20\%$  &  0.949 +/- 0.023 & 0.793 +/- 0.066 \\

 \hline
\end{tabular}
\end{table}
\end{center}



\begin{center}
\begin{table}[t]
\caption{Results of experiment I using the expanded adjacency matrix}
\label{tab:experiment1b}
\begin{tabular}{@{} *5l @{}}    \toprule
\emph{\% of anomalies (AN)} & \emph{AUC ROC} & \emph{AP} \\\midrule
$1\%$  &  0.931 +/- 0.016 & 0.513 +/- 0.050 \\
$5\%$  &  0.958 +/- 0.014 & 0.682 +/- 0.068 \\
$10\%$  &  0.975 +/- 0.008 & 0.785 +/- 0.053 \\
$15\%$  &  0.969 +/- 0.015 & 0.810 +/- 0.037 \\
$20\%$  &  0.978 +/- 0.008 & 0.826 +/- 0.048 \\

 \hline
\end{tabular}
\end{table}
\end{center}

% \begin{figure}
% 	\centering
% 		\includegraphics[scale=.55]{figs/roc_qtd.png}
% 	\caption{ROC curve for different quantities of anomalies.}
% 	\label{fig:roc_1}
% \end{figure}

% \begin{figure}
% 	\centering
% 		\includegraphics[scale=.55]{figs/pr_qtd.png}
% 	\caption{Precision-recall curve for different quantities of anomalies.}
% 	\label{fig:pr_1}
% \end{figure}



\subsection{Experiment II}\label{subsec:experiment2}

The second experiment compares the accuracy of \textit{SpecF} considering different anomaly intensities and keeping $AN$ fixed at 5\%. This experiment was carried out using the same network employed in the experiment described in Section \ref{subsec:experiment1}. Table \ref{tab:experiment2} reports the results of \textit{SpecF} when the standard adjacency matrix is used. In cases where the anomaly is extremely hard to identify, as in cases where the value of the signal at the anomalous nodes are only 1\% greater than the maximum signal in their community, the accuracy of the model is poor. In the case with anomaly intensity $\theta = 1\%$, for example, the value of PR was only 0.43, which is very close to the values obtained by a random classifier. Table \ref{tab:experiment2b} presents the results of this experiment using the expanded adjacency matrix $W$ instead. Again, the use of the matrix $W$ improves the results in anomaly detection in all scenarios.

\begin{center}
\begin{table}[t]
\caption{Results of experiment II using the standard adjacency matrix}
\label{tab:experiment2}
\begin{tabular}{@{} *5l @{}}    \toprule
\emph{Anomaly intensity ($\theta$)} & \emph{Mean AUC ROC} & \emph{Mean AP} \\\midrule
 $1\%$ & 0.925 +/- 0.057 & 0.427 +/- 0.169 \\
 $5\%$  & 0.923 +/- 0.035 & 0.628 +/- 0.080 \\
 $10\%$  & 0.900 +/- 0.020 & 0.681 +/- 0.023 \\
 $15\%$  & 0.868 +/- 0.016 & 0.673 +/- 0.032 \\
 $20\%$  & 0.857 +/- 0.021 & 0.681 +/- 0.024 \\

 \hline
\end{tabular}
\end{table}
\end{center}



\begin{center}
\begin{table}[t]
\caption{Results of experiment II using the expanded adjacency matrix}
\label{tab:experiment2b}
\begin{tabular}{@{} *5l @{}}    \toprule
\emph{Anomaly intensity ($\theta$)} & \emph{Mean AUC ROC} & \emph{Mean AP} \\\midrule
 $1\%$ & 0.957 +/- 0.030 & 0.431 +/- 0.179 \\
 $5\%$  & 0.946 +/- 0.017 & 0.648 +/- 0.074 \\
 $10\%$  & 0.939 +/- 0.015 & 0.716 +/- 0.037 \\
 $15\%$  & 0.919 +/- 0.017 & 0.730 +/- 0.039 \\
 $20\%$  & 0.887 +/- 0.014 & 0.697 +/- 0.018 \\

 \hline
\end{tabular}
\end{table}
\end{center}



% \begin{figure}
% 	\centering
% 		\includegraphics[scale=.5]{figs/roc_tax.png}
% 	\caption{ROC curve for different anomaly intensities.}
% 	\label{fig:roc_2}
% \end{figure}

% \begin{figure}
% 	\centering
% 		\includegraphics[scale=.5]{figs/pr_tax.png}
% 	\caption{Precision-recall curve for different anomaly intensities.}
% 	\label{fig:pr_2}
% \end{figure}
 
\subsection{Experiment III}

In this experiment, we evaluate the performance of our anomaly detection strategy in multiple independent executions. For this, we generated a set of five artificial networks for each mixture parameter described in Table \ref{tab:parameters}, totaling 40 different networks. We also generate 10 different anomalous signals for each network using the generator proposed in Section \ref{subsec:gerador}, totaling 400 different signals. The goal of this experiment is to better analyze the behavior of \textit{SpecF} considering a higher number of networks. We apply the anomaly detection technique to each of the 400 generated signals and calculate the average values of AUC-ROC and AP. This experiment was carried out for different values of network sizes ($n$), percentages of anomalies ($AN$), anomaly intensities ($\theta$) and adjacency matrices ($M$). The results are presented in Tables \ref{tab:experiment3.1} and  \ref{tab:experiment3.2}. In all cases, better results are obtained when the expanded adjacency matrix $W$ is used instead of the adjacency matrix $A$ in \textit{SpecF}.

%In this experiment \textcolor{blue}{we seek to evaluate the performance of the strategy in multiple independent executions. For this, we carry out ten independent executions with each combination of parameters in Table \ref{tab:parameters}}. \textcolor{red}{The goal is to better analyse} the behavior of the tool \textcolor{red}{considering a higher number of datasets}. 5 different networks were generated for each mixture parameter $\mu$ and ten independent runs were performed for each network, totaling 50 runs per $\mu$. We then calculated the average values of AUC-ROC and AP for this set of executions. This experiment was repeated by varying the size of the network ($n$), the percentage of anomalies ($AN$) and the intensity of the anomalies ($f$). The results of this experiment are illustrated in Figures \ref{fig:roc} and \ref{fig:ap}.

\begin{center}
\begin{table}[t]
\caption{Results of experiment III varying different parameters for $n = 500$}
\label{tab:experiment3.1}
\begin{tabular}{@{} *6l @{}}   \toprule
\emph{$n$} & \emph{$AN$}  & \emph{$\theta$}  & \emph{$M$}  & \emph{Mean AUC ROC}  & \emph{Mean AP}  \\\midrule
500 & 1\% & 1\% & $A$ & 0.756 +/- 0.16 & 0.170 +/- 0.15 \\
500 & 1\% & 1\% & $W$ & \textbf{0.956 +/- 0.04} & \textbf{0.339 +/- 0.18} \\\midrule
500 & 1\% & 5\% & $A$ & 0.797 +/- 0.15 & 0.233 +/- 0.18 \\
500 & 1\% & 5\% & $W$ & \textbf{0.971 +/- 0.03} & \textbf{0.492 +/- 0.21} \\\midrule
500 & 1\% & 10\% & $A$ & 0.847 +/- 0.12 & 0.322 +/- 0.21 \\
500 & 1\% & 10\% & $W$ & \textbf{0.990 +/- 0.02} & \textbf{0.712 +/- 0.22} \\\midrule
500 & 5\% & 1\% & $A$ & 0.740 +/- 0.11 & 0.286 +/- 0.13 \\
500 & 5\% & 1\% & $W$ & \textbf{0.947 +/- 0.02} & \textbf{0.550 +/- 0.11} \\\midrule
500 & 5\% & 5\% & $A$ & 0.780 +/- 0.11 & 0.356 +/- 0.14 \\
500 & 5\% & 5\% & $W$ & \textbf{0.970 +/- 0.02} & \textbf{0.715 +/- 0.12} \\\midrule
500 & 5\% & 10\% & $A$ & 0.836 +/- 0.09 & 0.463 +/- 0.16 \\
500 & 5\% & 10\% & $W$ & \textbf{0.985 +/- 0.02} & \textbf{0.836 +/- 0.13} \\\midrule
500 & 10\% & 1\% & $A$ & 0.714 +/- 0.12 & 0.364 +/- 0.13 \\
500 & 10\% & 1\% & $W$ & \textbf{0.931 +/- 0.02} & \textbf{0.631 +/- 0.09} \\\midrule
500 & 10\% & 5\% & $A$ & 0.763 +/- 0.11 & 0.444 +/- 0.14 \\
500 & 10\% & 5\% & $W$ & \textbf{0.958 +/- 0.02} & \textbf{0.758 +/- 0.09} \\\midrule
500 & 10\% & 10\% & $A$ & 0.815 +/- 0.09 & 0.529 +/- 0.13 \\
500 & 10\% & 10\% & $W$ & \textbf{0.975 +/- 0.02} & \textbf{0.855 +/- 0.10} \\
 \hline
\end{tabular}
\end{table}
\end{center}

\begin{center}
\begin{table}[t]
\caption{Results of experiment III varying different parameters for $n = 1000$}
\label{tab:experiment3.2}
\begin{tabular}{@{} *6l @{}}   \toprule
\emph{$n$} & \emph{$AN$}  & \emph{$\theta$}  & \emph{$M$}  & \emph{Mean AUC ROC}  & \emph{Mean AP}  \\\midrule
1000 & 1\% & 1\% & $A$ & 0.747 +/- 0.13 & 0.140 +/- 0.11 \\
1000 & 1\% & 1\% & $W$ & \textbf{0.951 +/- 0.03} & \textbf{0.292 +/- 0.13} \\\midrule
1000 & 1\% & 5\% & $A$ & 0.792 +/- 0.11 & 0.185 +/- 0.14 \\
1000 & 1\% & 5\% & $W$ & \textbf{0.970 +/- 0.03} & \textbf{0.444 +/- 0.18} \\\midrule
1000 & 1\% & 10\% & $A$ & 0.848 +/- 0.10 & 0.257 +/- 0.16 \\
1000 & 1\% & 10\% & $W$ & \textbf{0.984 +/- 0.02} & \textbf{0.614 +/- 0.21} \\\midrule
1000 & 5\% & 1\% & $A$ & 0.739 +/- 0.10 & 0.262 +/- 0.12 \\
1000 & 5\% & 1\% & $W$ & \textbf{0.944 +/- 0.02} & \textbf{0.543 +/- 0.10} \\\midrule
1000 & 5\% & 5\% & $A$ & 0.782 +/- 0.09 & 0.330 +/- 0.13 \\
1000 & 5\% & 5\% & $W$ & \textbf{0.963 +/- 0.02} & \textbf{0.672 +/- 0.13} \\\midrule
1000 & 5\% & 10\% & $A$ & 0.823 +/- 0.08 & 0.406 +/- 0.14 \\
1000 & 5\% & 10\% & $W$ & \textbf{0.979 +/- 0.02} & \textbf{0.793 +/- 0.14} \\\midrule
1000 & 10\% & 1\% & $A$ & 0.721 +/- 0.10 & 0.345 +/- 0.11 \\
1000 & 10\% & 1\% & $W$ & \textbf{0.927 +/- 0.02} & \textbf{0.623 +/- 0.08} \\\midrule
1000 & 10\% & 5\% & $A$ & 0.757 +/- 0.09 & 0.401 +/- 0.12 \\
1000 & 10\% & 5\% & $W$ & \textbf{0.954 +/- 0.02} & \textbf{0.742 +/- 0.10} \\\midrule
1000 & 10\% & 10\% & $A$ & 0.809 +/- 0.08 & 0.489 +/- 0.13 \\
1000 & 10\% & 10\% & $W$ & \textbf{0.970 +/- 0.02} & \textbf{0.825 +/- 0.11} \\

 \hline
\end{tabular}
\end{table}
\end{center}

% \begin{figure}
% 	\centering
% 		\includegraphics[scale=.27]{figs/compare.eps}
% 	\caption{AUC-ROC values for different mixture parameters.}
% 	\label{fig:roc}
% \end{figure}

% \begin{figure}
% 	\centering
% 		\includegraphics[scale=.27]{figs/compare_precision.eps}
% 	\caption{AP values for different mixture parameters.}
% 	\label{fig:ap}
% \end{figure}

Figure \ref{fig:mixture_types} illustrates the mean AP values for different values of $\mu$ and $\theta$ comparing the usage of matrices $A$ and $W$. It is evident that, in all cases, \textit{SpecF} performed better when it adopted matrix $W$ instead of matrix $A$. Besides, the results are better for larger values of $\theta$, as the anomalies are more evident. The primary weakness of \textit{SpecF} considering both matrices is apparently in cases where the anomaly is very slight and difficult to be identified.

% \begin{figure}
% 	\centering
% 		\includegraphics[scale=.6]{figs/output.png}
% 	\caption{Mean AP values for different values of $\mu$ and $\theta$.}
% 	\label{fig:mixture_types}
% \end{figure}

\begin{figure}[h!t]
\center

\input{tikz/output.tex}

\caption{Mean AP values for different values of $\mu$ and $\theta$.}
	\label{fig:mixture_types}
\end{figure}


% It is clear that in cases where the percentage of anomalies $AN$ is 5\%  and anomaly intensity $f$ is 5\%, the mean $AP$ values are less than 0.8, the case that the model achieved the worst accuracy. On the other hand, the best accuracy of the model was obtained in cases where $f$ was equal to 10\%, regardless of the number of anomalies in the network. This result shows that the primary weakness of the tool happens in cases where the anomaly is very slight and difficult to be identified. It is also evident that for $\mu > 0.4$, the mean AP values for cases where $f = 10\%$ are considerably higher than the mean AP values when $f = 5\%$ -- regardless of the amount $AN$ of anomalies being $5\%$ or $10\%$.

It is also worth noting that the anomaly detection strategy using the adjacency matrix $A$ presents worse results as the mixture parameter $\mu$ increases. In contrast, the performance improves as the value of $\mu$ increases when \textit{SpecF} employs matrix $W$. This behavior can be explained by the characteristics of the anomalous signal studied in this paper. We analyzed a signal whose anomaly is defined as a vertex whose value of the signal is different from that of the others in the same community. If the percentage of inter-community edges is low, the average signal values between communities are more distant. Therefore, even if the signal at a node differs from the community where it is located, it will still be closer to the average value of that community than to any other community's average value. When the mixture parameter is higher, the average values of the communities are closer. Moreover, a node whose signal value differs from the signal of its community may be close to the average values of neighboring communities. This characteristic is reflected in the Fourier transform through the expanded adjacency matrix and, then, demonstrated in the applied filter.

==> chapters/gsp.tex <==
Data from several applications can be represented by a graph $G = (V,E, A)$, where $V$ and $E$ are the sets of $n$ nodes and $m$ edges, respectively, and $A\in \mathbb{R}^{n\times n}$ is the weighted adjacency matrix. Each node $v_i\in V$ describes an instance of the dataset, and the weight $a_{ij}$ of an undirected\footnote{In this paper, we assume that $G$ is an undirected graph.} edge carries the strength of the relation between a pair of vertices $v_i$ and $v_j$. The degree of a vertex $v_i$ is quantified by the sum of the weights of the edges incident to it. The degree matrix $D\in\mathbb{R}^{n\times n}$ is the diagonal matrix whose $i^{th}$ diagonal
element $d_{ii}$ is equal to the degree of node $v_i$. Moreover, we denote here the set of neighbors of a vertex $v_i$ by $\mathcal{N}_i$, which means that this set contains all vertices adjacent to $v_i$.

%Opção 1: We represent a \textit{vertex signal} $\mathbf{f}: V \rightarrow \mathbb{R}$.%as a vector $\mathbf{f} \in \mathbb{R}^N$ where element $\mathbf{f}_i$ represents the signal value at node $v_i$\textcolor{red}{, i.e. $f(v_i)$}.
%\textcolor{red}{^n}

The graph signal, defined by function $f:V \rightarrow \mathbb{R}$, is represented by a vector $\mathbf{f} \in \mathbb{R}^n$, where each element $f_i$ corresponds to the signal of node $v_i\in V$, i.e, $f(v_i)$.%, 

\subsection{Graph Fourier Transform}\label{sec:fourier}

The graph Laplacian, also known as the non-normalized graph Laplacian, is defined by $L = D - A$, corresponding to a real-valued symmetric matrix. %%In GSP, $L$ can be understood as a difference operator, since:

%%$$
%%(Lf)(v_i)=\sum_{i\in \mathcal{N}_i}a_{ij}[f(v_i)-f(v_j)]
%%$$

 %As $L$ is a real symmetric matrix, it possesses a complete set of orthonormal eigenvectors. 
The eigenvectors of $L$ are orthonormal and have associated real and non-negative eigenvalues ${\{ \lambda_l \}}_{l=0, 1, ..., n-1}$\footnote{In this paper, we assume that $G$  has a single connected component.}, which we assume to be ordered as $ 0 = \lambda_0 < \lambda_1 \leq \lambda_2 ... \leq \lambda_{n-1} \coloneqq \lambda_{max}$.
 %The eigenvectors of $L$ are orthonormal and have associated real and non-negative eigenvalues ${\{ \lambda_l \}}_{l=0, 1, ..., n-1}$, which we assume to be ordered as $ 0 = \lambda_0 < \lambda_1 \leq \lambda_2 ... \leq \lambda_{n-1} \coloneqq \lambda_{max}$. 
 Let $U=[u_{ij}]_{n\times n}$ %where $u_{ij}\in \mathbb{R}$ 
 be the set of eigenvectors of $L$ organized in columns of $U$, according to the order of their corresponding eigenvalues. As $U$ is orthornomal, we have that $U^TU=I$.
%, denoted here by ${\{ \mathbf{u}_l \}}_{l = 0, 1, ..., n-1}$. \textcolor{red}{Parou aqui} -


 The graph Fourier transform $\hat{\mathbf{f}}$ of a signal $\mathbf{f} \in \mathbb{R}^n$ given a symmetric shift operator $S=R \Lambda R^*$ is $\hat{\mathbf{f}}=R^*\mathbf{f}$ \citep{Shuman2013}. As $L=U \Lambda U^T$, $U^*=U^T$, the graph Fourier transform given $L$ is calculated by $\mathbf{\hat{f}}=U^T\mathbf{f}$, known as  the expansion of $\mathbf{f}$ in terms of the eigenvectors of the graph Laplacian. In addition, the $l$-th row of $U^T$ corresponds to the eigenvector associated with $\lambda_l$ and each component of $\mathbf{\hat{f}}$ can be written as:

\begin{equation}\label{eq:fourier}
     \hat{f}(\lambda_l)  = \sum_{i=1}^{n} u_{il} f(v_i), \ \ \ \forall l\in \{0,\ldots,n-1\}
 \end{equation}

Let $\mathbf{i\hat{f}}=U\mathbf{\hat{f}}$ be the inverse graph Fourier transform of $\mathbf{\hat{f}}$ considering the same shift operator $L$. It is noteworthy that it is possible to return to the signal $\mathbf{f}$ by the inverse graph Fourier transform of $\mathbf{f}$, since $$\mathbf{i\hat{f}}=U\mathbf{\hat{f}}=U U^T\mathbf{f}=I\mathbf{f} = \mathbf{f}$$ Therefore, we have that

\begin{equation}\label{eq:inversefourier}
     f(v_i)  = \sum_{l=0}^{n-1} u_{il} \hat{f}(\lambda_l), \ \ \ \forall i\in \{1,\ldots,n\}. 
 \end{equation}

% is given by $U\mathbf{\hat{f}}$
% ANTIGO
% Analogously to classical Fourier transform, the graph Fourier transform $\hat{\mathbf{f}}$ of a signal $\mathbf{f} \in \mathbb{R}^n$ on the vertices of $G$ is defined as the expansion of $\mathbf{f}$ in terms of the eigenvectors of the graph Laplacian \citep{Shuman2013}:

% \begin{equation}\label{eq:fourier}
%     \hat{f}(\lambda_l) \coloneqq \langle \mathbf{f}, \mathbf{u}_l \rangle = \sum_{i=1}^{N} f(v_i) u_{l}^{*}(i)
% \end{equation}


% \noindent and the inverse graph Fourier transform is then given by

% \begin{equation}\label{eq:inversefourier}
%     f(i) = \sum_{l=0}^{N-1} \hat{f}(\lambda_l)u_{l}(i)
% \end{equation}
% ANTIGO TERMINA AQUI

\subsection{Frequencies on Graphs}

%In classical Fourier analysis, the eigenvalues \textbf{$\{(2\pi\xi)^2\}$} \textcolor{red}{of the eigenfunctions $\{(2\pi\xi)^2 e.....\}$} carry the notion of high and low frequencies. 
%low frequencies are associated with smooth complex exponential eigenfunctions that slowly oscillate, whereas high frequencies are related to complex exponential eigenfunctions that oscillate much more rapidly. 

In classical Fourier analysis, eigenvalues \textbf{$\{(2\pi\xi)^2\}$} carry the notion of high and low frequencies. Low frequencies are associated with smooth complex exponential eigenfunctions that slowly oscillate, whereas high frequencies are related to complex exponential eigenfunctions that oscillate more rapidly. 

In graph Fourier analysis, the graph Laplacian eigenvectors associated with small eigenvalues $\lambda_l$ vary slowly across the graph vertices, whereas  eigenvectors associated with larger eigenvalues oscillate more rapidly. It means that if two vertices are connected by an edge with a large weight, the values of the eigenvector at those locations are likely to be similar. This concept is then used to define low frequencies and high frequencies for signals indexed by graphs, represented by the Laplacian eigenvalues. 

%Lf =U\sigma U^T f=U \sigma f*
%Lf = \sigma f, since f is 
\subsection{Low-Pass Graph Filter}\label{sec:filter}

Frequency filtering is the process of representing an input signal as a linear combination of complex exponentials. As a consequence, filtering amplifies or attenuates the contributions of some frequencies. Graph spectral filtering can be directly generalized as

\begin{equation}\label{eq:filtro}
    f_{out}(\lambda_l) = f_{in}(\lambda_l)h(\lambda_l)
\end{equation}

\noindent where $h(\bullet)$ is the transfer function of the filter and  $f_{in}$ is the Fourier transform of an input signal function.  Several well-known continuous filtering techniques can be implemented as discrete, considering filtering functions that satisfy Equation \eqref{eq:filtro}, such as Gaussian smoothing, bilateral filtering, total variation filtering, anisotropic diffusion, and non-local means filtering \citep{Buades2005a}.

We call filters low-pass if they do not significantly affect the frequency content of low-frequency signals but attenuate the magnitude of high-frequency signals. An ideal low-pass filter keeps the magnitude of the spectrum at low frequencies unchanged and attenuates it at high frequencies. The frequency response of these filters is defined as

\begin{equation}
    h(\lambda_l)= \alpha_l = 
    \begin{cases}
      1, & \lambda_l < \lambda_{cut} \\
      0, & \lambda_l \geq \lambda_{cut}
    \end{cases}
  \end{equation}
  
\citet{Sandryhaila2014} demonstrated that the design of these filters is a linear problem and the construction of a filter with frequency response $h(\lambda_l) = \alpha_l$ corresponds to solving a system of $n_l$ non-linear equations:

\begin{align*}
  h_0 + h_1\lambda_0 + ... + h_{d_p}\lambda_0^{d_p}=& \,\alpha_0, \\ 
  h_0 + h_1\lambda_1 + ... + h_{d_p}\lambda_1^{d_p}=& \,\alpha_1, \\ 
  \vdots\\
  h_0 + h_1\lambda_{n_l-1} + ... + h_{d_p}\lambda_{n_l-1}^{d_p}=& \,\alpha_{n_l-1}
\end{align*}

\noindent where $d_p$ is the degree of the polynomial. We can find an approximate solution by, for example, the least squares method, to get around the over-determination of the system when $n_l \geq {d_p} + 1$.

==> chapters/introduction.tex <==
The explosive growth of technology has led to a substantial increase in the amount of data collected from several applications. They include sensor measurements, transportation, internet, biological data, financial transactions, among others. Data analysis and processing techniques to manage massive amounts of data are, therefore, of paramount importance.  Data generally have an irregular structure \citep{Newman2010} and a usual way of representing relational data is through graphs.  

%The  huge amount of data collected every day requires techniques capable of efficiently process and analyze.
Several techniques have been developed over the last years to analyze graphs. Generally, these techniques extract structural properties of networks to obtain relevant information about the data, such as node centrality, degree distribution, clustering, community structure, etc. \citep{Lancichinetti2009, Boccaletti2006, Schaeffer2007}. Nonetheless, these techniques usually end up exploring only the relational properties and not the data themselves.

Graph signal processing (GSP) techniques extend concepts from classical signal processing to signals indexed by generic graphs \citep{AliakseiSandryhaila2013, Shuman2013} and seek to analyze the data considering its underlying relational structure. Data from various domains can be modeled as graph-indexed signals, such as sensor networks, molecular network interactions, financial transaction data, among others. For example, graphs can represent data collected from sensor networks, where sensors correspond to vertices, and edges connect sensors close to each other. The signals on the graph nodes correspond to the set of values measured by the sensors at a given time. Thus, GSP tools are used for many purposes, such as fault diagnosis, signal denoising, signal compressing, and anomaly detection \citep{Chen2014, Shuman2013,gao2021fault}.

%Graph signal processing (GSP) techniques extend concepts from classical signal processing to signals indexed by generic graphs \citep{AliakseiSandryhaila2013, Shuman2013} and seek to analyze the data considering \textcolor{red}{its underlying} relational structure. Graph-indexed signals can be obtained from several applications, such as sensor networks, molecular network interactions, financial transaction data, among others. For example, data collected from sensor networks can be modeled as a graph where sensors are represented by  vertices and edges connect sensors which are close to each other. The set of values measured by the sensors at a given time can be seen as signals indexed by the vertices of this graph. Thus, GSP tools can be used to many purposes, such as signal denoising, signal compressing and anomaly detection \citep{Chen2014, Shuman2013}.

Two approaches are commonly employed for processing signals indexed by graphs. The first considers the Laplacian matrix and is based on the spectral graph theory \citep{ChungFanRKandGraham1997,nascimento2011spectral}. The second relies on the adjacency matrix and is based on algebraic signal processing theory \citep{Puschel2008, Puschel2008a}. Both approaches generalize classical signal processing operations, such as filtering and Fourier transform, to the graph domain, by defining the concept of graph filters and graph Fourier transform, respectively \citep{Sandryhaila2014}. 

Laplacian-based methods emerged from research on spectral graph theory and use the eigendecomposition of a particular representation of the graph, known as Laplacian matrix or graph Laplacian. The spectrum of the graph Laplacian provides the notion of frequencies in the graph Fourier transform. Laplacian matrices are symmetric and semi-definite positive when defined by symmetric adjacency matrices (undirected graphs), which means that graph Laplacian eigenvalues are real and orderable. %As with time-defined signals, \textcolor{red}{frequency spectra} the notions of high and low frequencies can be defined in graph signals. However,  due to the positive symmetry and semi-definition of the operator, Laplacian-based methods are only applicable to undirected graphs with non-negative real weights \citep{Shuman2013TheDomains, EkambaramCIRCULANTPROCESSING}.
%which is a strategy that uses a low-passfilter to attenuate the magnitude of the high frequencies of the spectrumˆfofa signalf. 
% The frequencies are the eigenvalues of the Laplace operator and the operator is symmetrical and semi-defined positive, leading to real and orderable frequencies. graph Laplacian matrices for frequency analysis of graph signals. the notions of high and low frequencies

This paper proposes a method to detect anomalies in signals indexed by graphs using GSP theory and spectral graph theory.  In comparison to the related literature, the introduced method, called \textit{SpecF}, besides considering the adjacency relationships between vertices takes the community structure into account at the graph Fourier transform. This is achieved by incorporating the network community structure into an expanded adjacency matrix. It is possible to understand the expanded adjacency matrix as a modification of the original unweighted graph to a weighted network through the inclusion of new edges. The method marks vertices whose signal values are outside the expected behavior from the community they belong to as potential anomalies. 


Computational experiments comparing the accuracy of the novel method with a counterpart using the classical adjacency matrix evidence the superiority of our community detection-based strategy 
in recovering anomalies, even for the most discrete cases. We also show by the proposed strategy the anomalous growth in the number of COVID-19 cases in the different districts of an upstate city of São Paulo, Brazil, known as São José dos Campos. We highlight the main contributions of this paper next.


\begin{itemize}
  \item The proposed anomaly detection algorithm addresses attributed networks for which the literature is scarce of anomaly detection algorithms;
    \item The introduced anomaly detection algorithm, called \textit{SpecF}, is  based on graph signal processing theory and defines anomalous objects as those nodes whose signals required the most significant correction by a low-pass filter;
     \item \textit{SpecF} differs from  other community-based anomaly detection methods by explicitly using the community structure in an extended adjacency matrix; 
    \item For a better assessment of the proposed framework, we introduce a methodology to add normal and anomalous signals to networks with community structure;
    \item We apply \textit{SpecF} to COVID-19 data to analyze the dissemination of the COVID-19 virus by investigating the anomalous districts of an upstate city from Brazil with approximately 730 thousand inhabitants.
\end{itemize}

% DESTACAR
% [08:58, 12/30/2020] Rodrigo: em sinais tipo o do zelanis
% [08:58, 12/30/2020] Rodrigo: onde a variação do sinal para nós dentro de uma mesma comunidade é esperada que seja similar
% [08:58, 12/30/2020] Rodrigo: e não somente vizinhos
% [08:59, 12/30/2020] Rodrigo: uma rede com indice de mistura maior por ex, se vc usar a adj só, os vizinhos pertencerão a varias comunidades diferentes
% [08:59, 12/30/2020] Rodrigo: e analisar só essa vizinhança na transformada pode deixar as coisas confusas
% [08:59, 12/30/2020] Rodrigo: uma vez que a variação dos nós dentro da comunidade é esperada que seja similar
% [09:00, 12/30/2020] Rodrigo: dados com estrutura de comunidades + um sinal que varia de forma similar para nós de uma mesma comunidade

==> chapters/related.tex <==
%that go out of expected
An important task in data mining is to find instances with unexpected behavior, which are more likely to be anomalous instances. Although several techniques have been developed over the last years to identify anomalies in data \citep{li2021clustering}, there are few techniques capable of efficiently dealing with graph-structured data. Graph structured data have complex correlations and require techniques capable of analyzing not only the data itself but the relations between the elements. In particular, we are interested in graphs with node attributes to find community outliers. A community outlier is a node whose attribute values deviate significantly from its community members.

% ANTIGO
%In a recent survey on graph-based anomaly detection, \citeauthor{Akoglu2015GraphSurvey} pointed out only two community-based methods for detecting anomalies in graphs with attributes. The first, introduced by \citeauthor{GaoOn}, is a probabilistic model that characterizes both data and links simultaneously. They propose to consider both structural information from the network and data information to find more meaningful outliers. According to the authors, the algorithm, called community outlier detection algorithm (CODA), is able to identify meaningful community outliers. The second method is a node outlier ranking technique in attributed graphs, called GOutRrank, developed by  \citeauthor{Muller2013}. GOutRrank ranks the graph nodes according to their degree of deviation in both graph-relational data and node attribute properties. 

In a recent survey on graph-based anomaly detection, \citeauthor{Akoglu2015GraphSurvey} pointed out only two community-based methods for detecting anomalies in graphs with attributes. The first, introduced in \citep{GaoOn}, is a probabilistic model that considers both relational and raw data information to find more meaningful outliers. On the one hand, the information regarding the relation is obtained from the topological structure of the network and describes the relationships that exist between instances of the dataset. On the other hand, the network node attributes store the data. According to the authors, the algorithm, called community outlier detection algorithm (CODA), can identify meaningful community outliers. The second method is a node outlier ranking technique in attributed graphs, called GOutRank, developed by   \cite{Muller2013}. GOutRank ranks the graph nodes according to their degree of deviation in both graph-relational data and node attribute properties. 

In a particular case of attributed graphs, where the attributes of the nodes can be interpreted as a signal indexed by the graph, techniques that extend signal processing concepts to the graph domain can be used to identify anomalies. For example, attributed graphs can represent wireless sensor networks, where each (sensor) node stores the value measured by the corresponding sensor in an instant of time. In this case, to identify an anomaly, it is necessary to consider the geographical proximity between the sensors and the values sensed by them. A sensor measurement significantly different from neighboring sensors' represents a potential anomaly. For this type of application, classical signal processing techniques, such as filters, can be extended to the graph domain.

Several studies use graph-based filters for data compression, data recovery, classification, noise removal, signal recovering, among others. However, to the best of our knowledge, few studies have adopted graph-based filtering to detect anomalies. \cite{Sandryhaila2014}, for example, introduced the concept of total variation to frequency sorting. The authors developed a filter using the proposed ordering method to identify malfunctions in sensor networks by extracting high-frequency components.  \cite{Qualcomm2014SpectralGraphs} introduced a spectral anomaly detection method that also uses a graph-based filter. They considered collective anomalies which occurred locally in time and space and applied the proposed method to sensor networks. 

%\citeauthor{Sharpnack2016DetectingStatistic} also propose an anomaly detection method using a low-pass filter based on the graph Fourier transform.

%The aforementioned studies employs concepts of classical signal processing theory, such as filters, to  the anomaly detection task. 
Both \cite{Sandryhaila2014} and \cite{Qualcomm2014SpectralGraphs}  adopted spectral filters and presented experiments with sensor network data where the adjacency relationships may be sufficient to detect nodes whose attributes deviate from the attributes of other nodes from the same community. However, in applications where the adjacency relationships are not only based on the physical distance, identifying a community outlier may consider the network's community structure. Neither of the previous work takes such information into account in their analysis. 

In protein-protein interaction networks, for example, adjacency relationships define the biological strength of the interaction between a pair of proteins. Proteins, represented by the graph nodes, may have quantitative attributes that correspond to the expression level of the protein in the network. In these networks, a community can be interpreted as a group of functionally related proteins \citep{Francisquini2020} whose attributes have similar characteristics. For this type of application, analyzing only the adjacency affinities may not reveal relevant information. Then, the data analysis must consider the community structure explicitly. To the extent of our knowledge, there is no graph-based filter method to detect anomalies that also takes the community structure into account, as proposed here.
